Hello Again! LLM-powered Personalized Agent for Long-term Dialogue

Open-domain dialogue systems have seen remarkable advancements with the development of large language models (LLMs). Nonetheless, most existing dialogue systems predominantly focus on brief single-session interactions, neglecting the real-world demands for long-term companionship and personalized interactions with chatbots. Crucial to addressing this real-world need are event summary and persona management, which enable reasoning for appropriate long-term dialogue responses. Recent progress in the human-like cognitive and reasoning capabilities of LLMs suggests that LLM-based agents could significantly enhance automated perception, decision-making, and problem-solving. In response to this potential, we introduce a model-agnostic framework, the Long-term Dialogue Agent (LD-Agent), which incorporates three independently tunable modules dedicated to event perception, persona extraction, and response generation. For the event memory module, long and short-term memory banks are employed to separately focus on historical and ongoing sessions, while a topic-based retrieval mechanism is introduced to enhance the accuracy of memory retrieval. Furthermore, the persona module conducts dynamic persona modeling for both users and agents. The integration of retrieved memories and extracted personas is subsequently fed into the generator to induce appropriate responses. The effectiveness, generality, and cross-domain capabilities of LD-Agent are empirically demonstrated across various illustrative benchmarks, models, and tasks. The code is released at https://github.com/leolee99/LD-Agent.

==> chapters/0_abstract_pre.tex <==
\begin{abstract}
Open-domain dialogue systems have seen remarkable advancements with the development of %pre-trained 
large \dy{language} models (LLMs). 
Nonetheless, most existing \za{dialogue
systems} predominantly focus on brief single-session interactions, neglecting the real-world demands for long-term companionship and personalized interactions with chatbots. 
% Event summary and personas are two crucial factors in reasoning appropriate responses in long-term dialogue. 
\za{Crucial to addressing this real-world need are event summary and persona management, which enable reasoning for appropriate long-term dialogue responses.}
\za{Recent progress in the human-like cognitive and reasoning capabilities of LLMs suggests that LLM-based agents could significantly enhance automated perception, decision-making, and problem-solving.}
% Benefiting from the excellent human-like cognitive and reasoning capabilities of large language models, LLM-based agents have become a prevalent solution for automated perception, decision-making, and problem-solving. 
\za{In response to this potential, we introduce a model-agnostic framework, the \underline{L}ong-term \underline{D}ialogue \underline{Agent} (\textbf{LD-Agent}), which incorporates three independently tunable modules dedicated to event perception, persona extraction, and response generation.}
% In this work, we introduce a model-agnostic \underline{L}ong-term \underline{D}ialogue \underline{Agent} framework, named LD-Agent, incorporating three independently tunable modules dedicated to event perception, persona extraction, and response generation. 
For the event memory module, long and short-term memory banks are employed to separately focus on historical and ongoing sessions, while a topic-based retrieval mechanism is introduced to enhance the accuracy of memory retrieval. 
Furthermore, the persona module conducts dynamic persona modeling for both users and agents. 
The integration of retrieved memories and extracted personas is subsequently fed into the generator to induce appropriate responses. 
The effectiveness, generality, and cross-domain capabilities of LD-Agent are empirically demonstrated across various illustrative benchmarks, models, and tasks. The code is released at \url{https://anonymous.4open.science/r/LDA-D7B6}.

\end{abstract}

==> chapters/1_introduction_pre.tex <==
\section{Introduction}
\label{sec:introduction}
Open-domain dialogue systems aim to establish long-term, personalized interactions with users via human-like chatbots~\cite{MSC, HAHT, DuLeMon}.
Unlike most existing studies~\cite{DailyDialog, PersonaChat, EmpatheticDialogues} that are limited to brief, single-session interactions spanning 2-15 turns, real-life scenarios often necessitate a chatbot's capability for long-term companionship and familiarity~\cite{MSC, HAHT, CC}.
Achieving this requires the chatbot not only to understand and remember extensive dialogue histories but also to faithfully reflect and consistently update both the user's and its personalized characteristics~\cite{MSC, CC, GapChat}.


% Open-domain dialogue is a promising research topic that aims to deploy human-like chatbots to fulfill daily conversational needs. 
% Most studies~\cite{DailyDialog, PersonaChat, EmpatheticDialogues} focus predominantly on one-time dialogues, confined to single sessions of just 2-15 turns. 
% In contrast, real-life scenarios often require a dialogue agent capable of providing long-term companionship and developing familiarity, rather than initiating each conversation as though with a stranger. 
% Consequently, there is an urgent and significant demand for long-term dialogue~\cite{MSC, CC, GapChat} to establish and maintain enduring, personalized relationships with users.

Motivated by real-life demands, the core challenge of open-domain dialogue systems is to simultaneously maintain long-term event memory and preserve persona consistency~\cite{DIM, D3, UniMC, DuLeMon}.
Existing research often addresses these aspects separately—focusing either on event memory or persona extraction—thereby hindering long-term consistency.
Current strategies for event memory typically involve constructing a memory bank that stores historical event summaries, complemented by retrieval-augmented approaches to access relevant information for response generation~\cite{MemNN, MAD}. 
Studies on persona-based dialogue rang from unidirectional user modeling~\cite{ORIG} to bidirectional agent-user modeling~\cite{PAG, P2, DuLeMon}, enhancing personalized chat abilities by leveraging profile information. 
Worse still, the aforementioned methods are highly dependent on specific model architectures, making them challenging to adapt to other models. Additionally, These dialogue models largely lack zero-shot generalization capabilities, essential for effective deployment across various real-world domains~\cite{HAHT, DuLeMon}.
We conjecture that an optimal long-term dialogue framework should be model-agnostic, deployable in various real-world domains, and capable of autonomously integrating comprehensive data from both event memories and personas, as illustrated in Figure \ref{fig:Fig-Intro}.
% Worse still, these dialogue models largely lack zero-shot generalization capabilities, essential for effective deployment across various real-world domains~\cite{HAHT, DuLeMon}.
% We conjecture that an optimal long-term dialogue framework should be model-agnostic, capable of autonomously integrating comprehensive data from both event memories and personas, as illustrated in figure \ref{Fig-Intro}.
However, developing such a model-agnostic, cross-domain, and autonomous framework remains unexplored and challenging.


% The challenges of long-term dialogue tasks primarily involve two aspects: maintaining event memory~\cite{MemNN, MAD} and preserving persona consistency~\cite{ORIG, PAG, P2, DuLeMon}. 
% A typical paradigm~\cite{MemNN, MAD} for maintaining event memory involves constructing a memory bank to store historical event summaries, complemented by retrieval-augmented approaches to access relevant information for response generation. 
% In terms of persona consistency, some efforts have explored both unidirectional user modeling~\cite{ORIG} and bidirectional agent-user modeling~\cite{PAG, P2, DuLeMon}. Figure.~\ref{fig:Fig-Intro} illustrates an ideally updated long-term dialogue framework that incorporates comprehensive information, including event memory and personas. 
% Nonetheless, existing studies~\cite{MemNN, MAD, ORIG, PAG, P2, DuLeMon} typically focus on either events or personas independently, impeding the comprehensive achievement of long-term consistency. 
% Moreover, the reliance on model-specific frameworks severely limits the ability to automatically adapt to diverse scenarios.

\begin{figure*}[t]
    \centering    
    \includegraphics[width=0.9\linewidth,trim=50 185 50 185,clip]{Figures/Intro-Figure.pdf}
    \caption{
    The illustration of how event memory and personas guide long-term dialogue. 
    The event summary and personas are extracted from a conversation that occurred one week ago. In today's interaction, the event memory prompts the girl to inquire about the swimming lesson they scheduled last week. The personas, indicating that she is careful and professional in swimming, guide her to offer detailed and professional advice.
    }
    \label{fig:Fig-Intro}
\end{figure*}


Benefiting from the excellent human-like cognitive and reasoning abilities of large language models (LLM), there is an increasing trend~\cite{Mind2Web, Voyager, ChatDev, GenerativeAgent, Agent4Rec} to employ LLMs as the cores of agent-based simulation systems to automate the process of perception, decision-making, and problem-solving. While recent studies have developed LLM-powered agents in various fields, such as economics~\cite{SocioDojo}, politics~\cite{WarAgent}, sociology~\cite{Sociology}, and recommendation~\cite{Agent4Rec}, its application in open-domain dialogue remains unexplored. 
% Moreover, ensuring long-term consistency and achieving robust cross-domain capabilities in open-domain dialogue are significant challenges. 
To effectively support long-term open-domain dialogue, an LLM-powered dialogue agent framework should exhibit broad generality, cross-domain adaptability, and the ability to dynamically refine information across dimensions like events, user personalities, and agent personalities.

% Benefiting from the excellent comprehension and reasoning capabilities of large language models (LLM), LLM-powered agents have achieved remarkable advancements~\cite{Mind2Web, Voyager, PsyAgent, Rehearsal, S3} in automated perception, decision-making, and problem-solving. Recent studies~\cite{GenerativeAgent, ChatDev, Agent4Rec} employ memory modules to store summaries of historical events, but the ignorance of in-process personality modeling and updating impedes long-term dialogue performance. Furthermore, due to the complexity of the LLM-based agent framework and the heavy reliance on the zero-shot capabilities of LLMs, optimizing for specific dialogue tasks becomes extremely challenging.


In this paper, we propose \textbf{LD-Agent}—a model-agnostic \textbf{L}ong-term \textbf{D}ialogue \textbf{Agent} framework consisting of three \za{principal} components: an event memory perception module, a persona extraction module, and response generation module \za{(see the framework of LD-Agent in Figure \ref{fig:Framework})}. 
The event memory perception module is designed to enhance coherence across sessions by separately maintaining long-term and short-term memory banks. The long-term memory bank stores vector representations of high-level event summaries from previous sessions, refined through a tunable event summary module. 
The short-term memory bank \za{maintains} contextual information for ongoing conversations.
\za{The persona extraction module, designed to facilitate personalized interactions, incorporates a disentangled, tunable mechanism for accurate user-agent modeling.}
% Designed to enable personalized interactions, the persona extraction module incorporates a disentangled, tunable mechanism for accurate user-agent modeling. 
Extracted personas are continuously updated and \za{stored} in a long-term persona bank. 
These personas, along with relevant memories, \za{are then} integrated into the response generation module, guiding the generation of appropriate responses, as depicted in Figure~\ref{fig:Fig-Intro}.


We conduct comprehensive experiments \za{on} two illustrative long-term multi-session daily dialogue datasets, MSC~\cite{MSC} and Conversation Chronicles (CC)~\cite{CC}, to evaluate the effectiveness, generality, and cross-domain capabilities of the proposed framework.
In terms of effectiveness, \za{LD-Agent} achieves state-of-the-art performance on both benchmarks, significantly outperforming existing methods~\cite{HAHT, ChatGLM, Blenderbot}. 
\za{To assess generality, we examine the framework from both model and task perspectives.}
% We explore generality from both model and task perspectives.
From the model perspective, \za{LD-Agent is evaluated across a range of} both online and offline models, including LLMs~\cite{ChatGLM} and non-LLMs~\cite{Blenderbot}. 
% From the model perspective, we evaluate the framework on a variety of online and offline models, including both LLMs~\cite{ChatGLM} and non-LLMs~\cite{Blenderbot}. 
From the task perspective, we extend our evaluation to multiparty dialogue tasks~\cite{GSN}, where LD-Agent also demonstrates substantial improvements, showcasing its adaptability across different models and tasks.
% From the task perspective, we further assess the framework for multiparty dialogue tasks~\cite{GSN}. 
% The substantial improvements brought by LD-Agent across different models and tasks thoroughly demonstrate the framework's generality. 
Regarding the method's cross-domain capabilities, we design two cross-domain settings: tuning the model on the MSC dataset and testing it on the CC dataset, and vice versa. 
In both scenarios, \za{LD-Agent} shows competitive performance, \za{nearly matching the results of in-domain training.} 
% close to in-domain training.




% We conduct comprehensive experiments using two illustrative long-term multi-session daily dialogue datasets: MSC~\cite{MSC} and Conversation Chronicles (CC)~\cite{CC}. Our approach achieves state-of-the-art performance on both benchmarks, significantly outperforming existing methods. Furthermore, we evaluate our framework on a variety of online and offline models~\cite{Blenderbot, ChatGLM}, including zero-shot and tuned models, exhibiting the reliability and generalization of our framework. In parallel, we explore the distinctive contributions of the event memory and personas to long-term dialogue in detail. The impact of different types of retrieval methods and various persona extraction techniques on response generation has also been thoroughly investigated.

Our contributions can be summarized as follows:

% \begin{itemize}[leftmargin=*]
%     \item We develop LD-Agent, a general long-term dialogue agent framework, considering both historical events and personas. 
%     The event memory module ensures dialogue coherence across sessions, while the persona module ensures character consistency.
%     \item We introduce a disentangled, tunable approach for long-term dialogue to ensure the accuracy of each module. The highly modular framework enables it to adapt to various dialogue tasks through module re-training. 
%     \item We confirm the superiority of our proposed framework through rigorous experiments across multiple challenging benchmarks, diverse illustrative models, and various tasks. Extensive insightful ablation studies further highlight its effectiveness and generalization.
% \end{itemize}

\begin{itemize}[leftmargin=*]
    \item We develop LD-Agent, a general long-term dialogue agent framework, considering both historical events, ensuring  dialogue coherence across sessions, and personas, ensuring character consistency.%     
    % \item We develop LD-Agent, a general long-term dialogue agent framework, considering both historical events and personas. 
    %  The event memory module ensures dialogue coherence across sessions, while the persona module ensures character consistency.
    \item We introduce a disentangled, tunable approach for long-term dialogue to ensure the accuracy of each module. The highly modular framework enables it to adapt to various dialogue tasks through module re-training. 
    \item We confirm the superiority of our proposed framework through rigorous experiments across multiple challenging benchmarks, diverse illustrative models, and various tasks. Extensive insightful ablation studies further highlight its effectiveness and generalization.
\end{itemize}

==> chapters/2_related_work_pre.tex <==
\section{Related Work}
\label{sec:related_work}
\subsection{Long-term Open-domain Dialogue}
Open-domain dialogue aims to develop a human-like chatbot that can emulate human conversation, facilitating free-flowing dialogue on a wide range of topics. However, the dialogue's extent in earlier studies is often limited by conversation length, focusing primarily on brief conversations of about 2-15 turns within a single session~\cite{DailyDialog, PersonaChat, EmpatheticDialogues}. To support more realistic and extended conversations, a series of studies have explored the role of both external~\cite{Prophetic, Commonsense} and internal knowledge~\cite{HAHT, DuLeMon} on maintaining the feasibility of long-term dialogue. Commonly referenced external knowledge, such as commonsense~\cite{Commonsense}, medical~\cite{Medical}, and psychological~\cite{SoulChat} knowledge, serves as supplementary guidance for the reasoning process, ensuring logical coherence in extended contexts. In parallel, internal knowledge captured dynamically during long conversations generally contains historical events~\cite{MSC, GapChat, HAHT, CC} and personas~\cite{DIM, DuLeMon, D3, PAGE}. Historical events are typically summarized and stored into a memory bank to maintain dialogue coherence across sessions, while interlocutors' personas are maintained via a dynamic persona memory bank, which ensures character consistency in long-term conversations. In this study, we focus on the internal knowledge to integrate dynamically updated historical events and personas to conduct long-term personalized conversations.




% \subsection{Long-term Open-domain Dialogue}
% Open-domain dialogue aims to develop a human-like chatbot that can emulate human conversation, facilitating free-flowing dialogue on a wide range of topics. However, the dialogue's extent in earlier studies is often limited by conversation length constraints, focusing primarily on brief conversations of about 2-15 turns within a single session~\cite{DailyDialog, PersonaChat, EmpatheticDialogues}. To support the dynamics of more realistic and extended conversations, MSC dataset~\cite{MSC}, a resource characterized by multi-session dialogues that consist of approximately 50 turns over five distinct sessions is introduced. Afterward, remarkable advances in maintaining coherence over longer conversations have been made. HAHT~\cite{HAHT} implements an attention encoding mechanism designed to capture key historical information in protracted dialogues. Recently, the rapid development of LLMs has facilitated the advancement of long-term dialogue tasks, with some efforts~\cite{GapChat, CC} using LLMs to build multi-session datasets with expanded time intervals and longer gaps. However, achieving generalized long-term consistency in open-domain dialogues remains a substantial challenge. 
% %In this study, we introduce a historical memory retrieval framework designed to support multi-session long-term consistent dialogues.

% \subsection{Persona Dialogue}
% Persona dialogue is crucial for constructing consistent, human-like conversational systems. It typically involves extracting user profile from the dialogue, such as gender, age, and hobbies,~\etc. This personal attributes forms the foundation of a user persona database, which is instrumental in generating consistent conversational responses. A series of works~\cite{DIM, D3, PAGE, DuLeMon} have led to impressive successes in persona dialogue systems. Wu~\etal\cite{PAG} introduced personality-related characteristics of human dialogue into a variational response generator, thus guiding optimization towards the personalities of two characters. Liu~\etal\cite{P2} noticed the concept of mutual persona perception, proposing a transmitter-receiver framework for more accurate modeling of interlocutors. Chen~\etal\cite{ORIG} explored the impact of the persona input order on generation and designed a model-agnostic order insensitive generation framework. Recently, large language models showed strong capabilities on semantic understanding and problem solving, but often align with general, overall human preferences rather than individual ones, some studies~\cite{PSoups, ExploreLLM} have proposed predefined personalized response frameworks tailored to specific user preferences. 
%In this paper, we introduce a learnable dynamic user modeling framework that accurately extracts user profiles during prolonged user-agent interactions to facilitate more personalized responses.

\subsection{LLM-based Autonomous Agents}
AI Agent conception is geared towards autonomous environmental perception, decision-making, and problem-solving capabilities. With the large language models (LLMs) underlining their impressive generalization potential, leading to their widespread adoption as substitutes for human operators in various research fields~\cite{Mind2Web, ChatDev, PsyAgent, Agent4Rec}. Generally, these agents can be categorized into task-oriented agents~\cite{Mind2Web, Voyager, ChatDev, MemoryBank} and simulation-oriented agents~\cite{PsyAgent, Rehearsal, S3, Agent4Rec, RecAgent}. Task-oriented agents are designed to accurately perform and achieve predefined tasks, as seen in applications for web assistance~\cite{Mind2Web}, game-playing~\cite{Voyager}, and software development~\cite{ChatDev}. On the other hand, simulation-oriented agents are devised to emulate human emotive and cognitive behaviors, having played roles in psychological studies~\cite{PsyAgent}, social networking platforms~\cite{S3}, conflict resolution scenarios~\cite{Rehearsal}, and recommendation systems~\cite{Agent4Rec, RecAgent}. In addition, recent developments have seen the advent of individual-level agents that are utilized to simulate specific character behaviors, enhancing the realism and personalization of user-agent interactions~\cite{CharacterLLM, CharacterGLM, RoleLLM}. This paper falls into the simulation-oriented agent to build a human-like open-domain dialogue agent with memory retrieved and character analysis modules.

==> chapters/3_methodology_pre.tex <==
\section{Method}
\label{sec:method}
In this section, we introduce the LD-Agent in detail with the framework shown in Figure~\ref{fig:Framework}. We first introduce the task definition of long-term dialogue in Section.~\ref{sec:task}. Consequently, we separately introduce the mechanism of event perception (Section.~\ref{sec:event}), dynamic personas extraction (Section.~\ref{sec:persona}), and response generation (Section.~\ref{sec:response}).


\subsection{Task Definition}
\label{sec:task}
\za{
The goal of the long-term multi-session dialogue task is to generate an appropriate response $r$, by utilizing the context of the current session $C$, along with selected information extracted from historical session $H$.
In this task, the current conversation session $C$ is defined as $\{u_1,u_2,\dots,u_{d_c-1},u_{d_c}\}$, where each $u_i$ represents $i$-th utterance, and $d_c$ represents $d_c$ turns of the current session.
Each historical session within $H$ in $N$ historical sessions is denoted as $H^i$, containing $\{h^i_1, h^i_2, \dots, h^i_{d_i}\}$, where $d_i$ is the number of utterances of the $i$-th conversational session.
Distinct from single-session dialogue models, a long-term multi-session dialogue system integrates both current and long-term historical conversational cues to generate contextually appropriate responses. 
}

% For long-term multi-session dialogue task, $C=\{u_1,u_2,\dots,u_{d_c-1},u_{d_c}\}$ denotes $d_c$ turns context utterances of the current conversation session, where $u_i$ represents $i$-th utterance. $H=\{H^1, H^2, \dots, H^N\}$ denotes $N$ historical sessions, where $H^i=\{h^i_1, h^i_2, \dots, h^i_{d_i}\}$ denotes ${d_i}$ utterances of the $i$-th conversational session. The purpose of this task is to predict the appropriate agent response $r$ utilizing the context of the current session and limited information extracted from historical sessions $H$.

\subsection{Event Perception}
\label{sec:event}

The event memory module is designed to perceive historical events to generate coherent responses across interval time. 
As shown in Figure~\ref{fig:Framework}, 
\za{this event memory module is segmented into two major sub-modules that focus separately on long-term and short-term memory.}
% there are two major sub-modules to separately focus on long-term memory and short-term memory.
\begin{figure}[t]
    \centering    \includegraphics[width=0.5\textwidth,trim=160 140 160 140,clip]{Figures/Framework.pdf}
    \vspace{-5pt}
    \caption{The Framework of LD-Agent. The event module stores historical memories from past sessions in long-term memory and current context in short-term memory. The persona module dynamically extracts and updates personas for both users and agents from ongoing utterances, storing them in a persona bank for each character. The response module then synthesizes this data to generate informed and appropriate responses.}
    \label{fig:Framework}
\end{figure}

\subsubsection{Long-term Memory} 

\paragraph{Memory Storage.} 
The long-term memory module aims to \za{extract and encode} events from past sessions.
\za{Specifically, this involves recording the occurrence times $t$ and brief summaries $o$ into representations that are stored in a low-cost memory bank $M_L=\{\phi(t_j, o_j) \mid j \in \{1,2, \dots, l\}\}$.
Here, $\phi(\cdot)$ indicates the text encoder (\eg, MiniLM~\cite{MiniLM}), and $l$ specifies the length of the memory bank.
The encoded representations are then efficiently retrieved through an embedding-based mechanism, which enhances the accessibility of the stored memory. 
}


% encoding the occurrence times $t$ and brief summaries $o$ into representations that can be stored in a low-cost memory bank $M_L=\{\phi(t_j, o_j) \mid j \in \{1,2, \dots, l\}\}$, where $\phi(\cdot)$ indicates the encoder of MiniLM~\cite{MiniLM}, $l$ denotes the length of the memory bank. 
% These representations are efficiently retrieved through an embedding-based mechanism to enhance accessibility. 

\paragraph{Event Summary.}
Different from previous agent approaches~\cite{GenerativeAgent, Agent4Rec, MemoryBank} that entirely rely on LLM's zero-shot ability to excavate and summarize events, we apply instruction tuning~\cite{IT} to the event summary module, which can directly improve the event summary quality. 
Specifically, we rebuild the DialogSum dataset~\cite{DialogSum}, a large-scale dialogue summarization dataset, into the following format: (1) an introduction to the task background, (2) the related conversations that need to be understood, and (3) detailed summarization requests. 
These three parts serve as input prompts (see Appendix.~\ref{event_summary_prompt} for more details), combined with the original summaries from DialogSum as answers, and are jointly used to fine-tune the event summary module, \za{thereby directly improving the quality of event summarization.}

\paragraph{Memory Retrieval.} 
To improve retrieval accuracy, we employ a retrieval mechanism that comprehensively considers semantic relevance, topic overlap, and time decay. 
Optimizing the retrieval accuracy of agent memory is challenging due to the difficulty in obtaining accurate memory retrieval data. 
Most existing methods~\cite{GenerativeAgent, Agent4Rec} use event summaries as keys and context as queries, calculating the query-key semantic relevance score $s_{\text{sem}}$ to find relevant memories, which inevitably results in significant errors. 
To enhance retrieval reliability, we extract nouns from corresponding conversations with the summaries to construct a topic library $V$ and calculate topic overlap score $s_{\text{top}}$ by:
\begin{equation}
    s_{\text{top}}=\frac{1}{2}(\frac{\left | V_q\cap V_k \right |}{\left | V_{q} \right |}+\frac{\left | V_q\cap V_k \right |}{\left | V_{k} \right |}),
\label{eq:overlap_compute}
\end{equation}
where $V_q$, $V_k$ denote the topic noun set of query and key. Additionally, we apply a time decay coefficient $\lambda_t=e^{{-t}/{\tau}}$ to reweight the overall retrieval score $s_r$, signified as:
\begin{equation}
    s_{\text{overall}} = \lambda_t (s_{\text{sem}} + s_{\text{top}}).
\label{eq:retrieval_score}
\end{equation}
To avoid retrieving inappropriate memory due to no suitable memories existing, we implement a semantic threshold $\gamma$. Only memories with semantic score $s_\text{sem}$ greater than $\gamma$ could be retrieved. If no appropriate memories are retrieved, ``No relevant memory'' will be returned. 
Eventually, the process of retrieving relevant memory $m$ is denoted as:
\begin{equation}
    m = \psi(M_L, \gamma).
\label{eq:retrieval_function}
\end{equation}



\subsubsection{Short-term Memory} 
The short-term memory module actively manages a dynamic dialogue cache $M_S=\{(t_i,u_i)|i=\{1,2,3,\dots,r_c\}\}$ with timestamps to preserve the detailed context of the current session. 
Upon receiving a new utterance $u'$, the module first evaluates the time interval between the current time $t'$ and the last recorded time $t_{r_c}$ in the cache. 
If this interval exceeds a threshold $\beta$, the module triggers the long-term memory module to summarize the cached dialogue entries, creating new event records for storage in the long-term memory bank. 
Simultaneously, the short-term memory cache is cleared, and the new dialogue record $(t',u')$ is added to the cache. 
\za{The mathematical expression of this process is given by:}
\begin{equation}
    \begin{aligned}
    M'_L &= M_L \cup \{(\phi(t_{r_c}, A(M_S))\},\\
    M_S &= \{(t',u')\}.
    \end{aligned}
\label{eq:memory_update}
\end{equation}
where $M'_L$ denotes the updated long-term memory bank, $o=A(\cdot)$ is the event summary function, \za{which process the accumulated dialogue in $M_S$.}


\subsection{Dynamic Personas Extraction}
\label{sec:persona}
The persona module is pivotal in maintaining long-term persona consistency for both participants in a dialogue system. 
Drawing inspiration from prior work~\cite{DuLeMon}, we adopt a bidirectional user-agent modeling approach, utilizing a tunable persona extractor to manage long-term persona bank $P_u$ and $P_a$ for the user and agent, respectively. 
Specifically, we develop an open-domain, utterance-based persona extraction dataset derived from MSC~\cite{MSC}. 
%further details about this dataset can be found in Appendix~\ref{}. 
We enhance the persona extractor with LoRA-based instruction tuning, which allows for the dynamic extraction of personality traits during conversations. 
These traits are subsequently stored in the corresponding character's persona bank. 
For utterances devoid of personality traits, the module outputs ``No Trait''. 
%The tuned personas extractor is capable of directly integrating into multiparty tasks by simultaneously emulating multiple characters.
Additionally, we employ a tuning-free strategy that harnesses the zero-shot capabilities of LLM models to directly extract personas based on prompts (see Appendix.~\ref{persona_extraction_prompt}).  
To further improve the ability to excavate user personas without training, we adjust our reasoning strategy from direct reasoning to a Chain-of-Thought reasoning~\cite{CoT}.

\subsection{Response Generation}
\label{sec:response}
Upon receiving a new user utterance $u'$, the agent \za{integrates various inputs:} retrieved relevant memories $m$, short-term context $M_S$, and the personas $P_u$ and $P_a$ for the user and agent, respectively. 
\za{These combined inputs} are fed into a response generator to deduce an appropriate response \za{$r$}, formulated as
\begin{equation}
r=G(u',m,M_S,P_u,P_a).
\label{eq:response_generation}
\end{equation}
To enhance the agent's ability \za{for coherent and contextually appropriate responses},
% to generate reasonable responses, 
we develop a long-term, multi-session dialogue dataset, featuring dynamic retrieval memories, context, and personas sourced from the MSC and CC datasets for generator tuning. 
Specifically, for each sample, covering five sessions, we dynamically simulate the entire progression of the conversation. 
\za{As each new utterance is introduced,} the previously tuned modules for event summarization, persona extraction, and memory retrieval are utilized to collect the necessary context, retrieved memories, and both user and agent personas related to the utterance.
\za{This comprehensive data is then} integrated into a response generation prompt (see Appendix.~\ref{response_generation_prompt}). 
The original responses from the MSC and CC datasets are used as ground truth sentences.

==> chapters/4_experiments_pre.tex <==
\section{Experiments}
\label{sec:experimetns}
We aim to answer the following research questions:
\begin{itemize}[leftmargin=*]
   \item \textbf{RQ1:} How does LD-Agent perform in long-term dialogue tasks?
   %in out-of-distribution tasks? 
   \item \textbf{RQ2:} How is the generality and practicality of LD-Agent?

\end{itemize}

\subsection{Evaluation Settings}
In this subsection, we briefly introduce the experimental dataset, evaluation metrics, and baseline models in our study. Detailed evaluation settings are elaborated in Appendix.~\ref{sec:detailed_eval_settings}.


\paragraph{Datasets.} Extensive experiments are conducted on two illustrative multi-session datasets, \textbf{MSC}~\cite{MSC} and \textbf{CC}~\cite{CC}, each comprising 5 sessions with approximately 50 conversational turns per sample, to investigate the effectiveness of LD-Agent on long-term dialogue scenarios. The experiments cover model independence assessment, module ablation, persona extractor analysis, and cross-domain evaluation.
%We utilize these two benchmarks to investigate the effectiveness of LD-Agent on long-term dialogues through  model frameworks

Additionally, to evaluate the transferability of the LD-Agent, we apply our method to the \textbf{Ubuntu IRC benchmark}~\cite{GSN}, a dataset known for its multiparty interaction tasks.

% We utilize \textbf{MSC}~\cite{MSC} and \textbf{CC}~\cite{CC},  two illustrative multi-session datasets with 5 sessions and approximately 50 turns per conversation to validate the performance on Long-term dialogue. To explore the transferability of LD-Agent, we also apply our method to the \textbf{Ubuntu IRC benchmark}~\cite{GSN}, a dataset of multiparty task. 

\paragraph{Metrics.} 
Our evaluation combines both automatic and human assessments to thoroughly investigate the effectiveness of LD-Agent. For automatic evaluation, we use three widely used standard metrics: BLEU-N (BL-N)~\cite{BLEU}, ROUGE-L (R-L)~\cite{ROUGE}, and METEOR (MET)~\cite{METERO} to measure the quality of response generation. Additionally, accuracy (ACC) is employed to evaluate the classification performance of the persona extractor. In human evaluation, we measure topic coherence across sessions, interaction fluency, and user engagement using the metrics of coherence, fluency, and engagingness, respectively.

% We conduct automatic evaluation and human evaluation to comprehensive evaluate the effectiveness of LD-Agent. For automatic evaluation, three commonly used metrics, including BLEU-N (BL-N), ROUGE-L (R-L), and METEOR (MET), are utilized to measure the response generation quality, while accuracy (ACC) is utilized to measure the classification accuracy of different persona extractor. For human evaluation, coherence, fluency, engagingness are separately used to measure the interaction coherence across sessions, interaction fluency, and user's interests.

% We conduct our primary experiment using the Multi-Session Chat (MSC)~\cite{MSC} and CONVERSATION CHRONICLES (CC)~\cite{CC} datasets.The MSC dataset is a manually curated dialogue set collected through crowdsourcing. Each sample comprises five conversations, spaced by intervals of up to several days, and includes recordings of the participants' personas.The CC dataset is a collection of multi-session conversations generated by ChatGPT and structured around a predefined event graph.It defines the relationship between conversation participants (e.g. classmates, neighbors) and guides their interactions according to the event graph. Each sample comprises five sessions, each separated by time intervals that may extend over several years.

\paragraph{Baselines.}
To demonstrate the effectiveness and model independence of LD-Agent, we deploy LD-Agent on multiple platforms and models. Specifically, the LLM-based models (online model: ChatGPT; offline model: ChatGLM~\cite{ChatGLM}) and traditional language models (BlenderBot~\cite{Blenderbot}, and BART~\cite{BART}) are employed as our baselines. In our experiments, The notation ``\textbf{Model}\textsubscript{LDA}'' denotes models that incorporate the LD-Agent framework, while ``\textbf{Model}'' refers to the original baseline models without LD-Agent. Additionally, we also utilize HAHT~\cite{HAHT}, the previous state-of-the-art model in long-term dialogue task, as a contrast. See the above baselines stand and their role in rich literature in Appendix.~\ref{sec:related_work}.



% We compare the proposed agent model against the following baseline methods.

% \begin{itemize}
%     \item \textbf{H}istory-\textbf{A}ware \textbf{H}ierarchical \textbf{T}ransformer(\textbf{HAHT})~\cite{HAHT}: This is crafted for multi-session, open-domain dialogue, retaining a long-term memory of past conversations. This history informs its understanding of the current context, enabling it to generate responses that are both well-informed and relevant to the ongoing conversation.
%     \item \textbf{BlenderBot}~\cite{Blenderbot}: This is a large-scale, open-domain dialogue model that has been pre-trained using conversation data collected from online social discussions. On BlenderBot, we choose BlenderBot\_Samll-90M and finetune the prompts used for base and agent, respectively named: $\boldsymbol{{ \rm BlenderBot}_{base}}$ and $\boldsymbol{\rm BlenderBot_{agent}}$.
%     \item \textbf{BART}~\cite{BART}: This is a transformer-based model developed by Facebook for improving text understanding and generation. It's trained to reconstruct text from corrupted versions, which helps it perform well in tasks like summarization and translation.
%     \item \textbf{ChatGLM3}~\cite{ChatGLM}: This is a generation of pre-trained dialogue models jointly released by Zhipu AI and Tsinghua KEG. We choose ChatGLM3-6B model and deploy it locally.
%     \item \textbf{ChatGPT}: This is an AI language model developed by OpenAI, based on the GPT architecture. It is designed to generate human-like text responses in a conversational context. We use the API service provided by OpenAI, and the model selected is ``gpt-3.5-turbo-1106''.
% \end{itemize}

\begin{table*}[ht]
\centering
\captionsetup{skip=5pt}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{@{}clccc|ccc|ccc|ccc@{}}
\toprule
 & & \multicolumn{3}{c}{\textbf{Session 2}} & \multicolumn{3}{c}{\textbf{Session 3}} & \multicolumn{3}{c}{\textbf{Session 4}} & \multicolumn{3}{c}{\textbf{Session 5}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
\multicolumn{1}{c}{\multirow{-2}{*}{\textbf{}}} & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Model}}} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} \\
\midrule
\multicolumn{14}{c}{\textbf{MSC}}\\
\midrule
& ChatGLM & 5.44 & 1.49 & 16.76 & 5.18 & 1.55 & 15.51 & 5.63 & 1.33 & 16.35 & 5.92 & 1.45 & 16.63 \\
& ChatGLM\textsubscript{LDA} & 5.74 & 1.73 & 17.21 & 6.05 & 1.73 & 16.97 & 6.09 & 1.59 & 16.76 & 6.60 & 1.94 & 17.18 \\
& ChatGPT & 5.22 & 1.45 & 16.04 & 5.18 & 1.55 & 15.51 & 4.64 & 1.32 & 15.19 & 5.38 & 1.58 & 15.48 \\
\multirow{-4}{*}{\textbf{Zero-shot}} & ChatGPT\textsubscript{LDA} & 8.67 & 4.63 & 19.86 & 7.92 & 3.55 & 18.54 & 7.08 & 2.97 & 17.90 & 7.37 & 3.03 & 17.86 \\
\midrule
 & HAHT & 5.06 & 1.68 & 16.82 & 4.96 & 1.50 & 16.48 & 4.75 & 1.45 & 15.82 & 4.99 & 1.51 & 16.24 \\
 & BlenderBot & 5.71 & 1.62 & 16.15 & 8.10 & 2.50 & 18.23 & 7.55 & 1.96 & 17.45 & 8.02 & 2.36 & 17.65 \\
 & BlenderBot\textsubscript{LDA} & 8.45 & 3.27 & 19.07 & 8.68 & 3.06 & 18.87 & 8.16 & 2.77 & 18.06 & 8.31 & 2.69 & 18.19 \\
 & ChatGLM & 5.48 & 1.59 & 17.65 & 6.12 & 1.78 & 17.91 & 6.14 & 1.63 & 17.78 & 6.16 & 1.69 & 17.65 \\
\multirow{-5}{*}{\textbf{Tuning}}& ChatGLM\textsubscript{LDA} & \textbf{10.70} & \textbf{5.63} & \textbf{23.31} & \textbf{10.03} & \textbf{5.12} & \textbf{21.55} & \textbf{9.07} & \textbf{4.06} & \textbf{20.19} & \textbf{8.96} & \textbf{4.01} & \textbf{19.94} \\
\midrule
\multicolumn{14}{c}{\textbf{CC}}\\
\midrule
\multirow{4}{*}{\textbf{Zero-shot}} & ChatGLM & 8.94 & 4.44 & 21.54 & 8.34 & 4.03 & 21.00 & 8.28 & 3.82 & 20.67 & 8.12 & 3.81 & 20.54 \\
 & ChatGLM\textsubscript{LDA} & 9.53 & 4.82 & 22.76 & 9.22 & 4.43 & 22.18 & 9.15 & 4.48 & 22.18 & 8.99 & 4.43 & 22.10 \\
 & ChatGPT & 10.57 & 5.50 & 22.10 & 10.58 & 5.59 & 22.04 & 10.61 & 5.58 & 21.92 & 10.17 & 5.22 & 21.45 \\
 & ChatGPT\textsubscript{LDA} & 15.89 & 11.01 & 26.96 & 12.92 & 8.27 & 24.31 & 12.20 & 7.35 & 23.69 & 11.54 & 6.74 & 22.87 \\
\midrule
\multirow{4}{*}{\textbf{Tuning}} & BlenderBot & 8.99 & 4.86 & 21.58 & 9.44 & 5.19 & 22.13 & 9.46 & 5.21 & 22.08 & 8.99 & 4.75 & 21.73 \\
 & BlenderBot\textsubscript{LDA} & 14.47 & 10.16 & 27.91 & 15.66 & 11.33 & 29.10 & 15.13 & 10.80 & 28.38 & 14.08 & 9.72 & 27.37 \\
 & ChatGLM & 15.89 & 9.90 & 30.59 & 15.97 & 10.06 & 30.27 & 16.10 & 10.31 & 30.54 & 15.10 & 9.34 & 29.43 \\
 & ChatGLM\textsubscript{LDA} & \textbf{25.69} & \textbf{19.53 }& \textbf{39.67} & \textbf{25.93} & \textbf{19.72} & \textbf{39.15} & \textbf{25.82} & \textbf{19.40} & \textbf{39.05} & \textbf{24.26} & \textbf{18.16} & \textbf{37.61} \\
\bottomrule
\end{tabular}
}
\caption{Experimental results of the automatic evaluation for response generation on MSC and CC.}
\label{table:msc_cc}
\end{table*}


\subsection{Results of Multi-Session Dialogue}

We adopt two multi-session dialogue dataset to evaluate our method in long-term dialogue scenarios. The first session is used to initialize conversation and the subsequent four sessions are used to evaluate the performance of long-term dialogue. In these experiments, LD-Agent is applied to both zero-shot models, including ChatGLM and ChatGPT, and to tuned models like BlenderBot and ChatGLM with the results reported in Table~\ref{table:msc_cc}.
% To evaluate the effectiveness of our LD-Agent framework in multi-session dialogue, we conducted tests on two datasets: MSC and CC.
\paragraph{Impressive performance on long-term dialogue tasks.} On both datasets, all models employing LD-Agent consistently achieve significant improvements across all sessions and metrics, showcasing the powerful ability of LD-Agent on supporting long-term dialogue. Most notably, comparing with previous state-of-the-art model HAHT, BlenderBot employing LD-Agent, which has similar parameter scale to HAHT, outperforms it with a large performance gap of 3.39\%, 3.72\%, 3.41\%, and 3.32\% on BLEU-2 ranging from session 2 to 5. This further highlighting the effectiveness of LD-Agent on long-term dialogue tasks.


\paragraph{Remarkable generality of LD-Agent.} The generality of LD-Agent are proved from two aspects: data transferability and model transferability. The consistently improvements brought by LD-Agent on both benchmarks demonstrate the generality of our framework on various long-term dialogue scenarios. In parallel, we observe that LD-Agent also plays positive roles in the zero-shot setting, employing to the online model of ChatGPT and the offline model of ChatGLM. In the tuning setting, LD-Agent achieves significant enhancements on both LLM of ChatGLM and traditional model of BlenderBot, fully proving the remarkable model transferability of LD-Agent. These results comprehensive demonstrate the generality of LD-Agent. 

\begin{table*}[t]
\centering
\captionsetup{skip=5pt}

\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{@{}clccc|ccc|ccc|ccc@{}}
\toprule
 & & \multicolumn{3}{c}{\textbf{Session 2}} & \multicolumn{3}{c}{\textbf{Session 3}} & \multicolumn{3}{c}{\textbf{Session 4}} & \multicolumn{3}{c}{\textbf{Session 5}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
\multicolumn{1}{c}{\multirow{-2}{*}{\textbf{}}} & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Model}}} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} \\
\midrule
 & Baseline & 5.48 & 1.59 & 17.65 & 6.12 & 1.78 & 17.91 & 6.14 & 1.63 & 17.78 & 6.16 & 1.69 & 17.65 \\
 & + Mem & 7.57 & 2.49 & 19.50 & 7.70 & 2.48 & 19.46 & 7.53 & 2.31 & 19.26 & 7.56 & 2.33 & 19.03 \\
 & + Persona\textsubscript{ user} & 7.54 & 2.57 & 19.68 & 7.51 & 2.38 & 19.39 & 7.30 & 2.09 & 18.80 & 7.08 & 2.27 & 18.79 \\
 & + Persona\textsubscript{ agent} & 7.00 & 2.27 & 18.70 & 7.23 & 2.33 & 18.75 & 7.32 & 2.18 & 18.47 & 7.13 & 2.36 & 18.48 \\
 & Full & \textbf{10.70} & \textbf{5.63} & \textbf{23.31} & \textbf{10.03} & \textbf{5.12} & \textbf{21.55} & \textbf{8.96} & \textbf{4.01} & \textbf{19.94} & \textbf{9.07} & \textbf{4.06} & \textbf{20.19} \\
\bottomrule
\end{tabular}
}
\caption{Ablation study results of LD-Agent on MSC. The experiments are conducted on tuned ChatGLM. 
Baseline denotes the model tuned with context of current session. ``+ module name'' indicates the model tuned solely with context and corresponding module. ``Full'' indicates the model tuned with all modules.} 
\label{table:msc_ablation}
\end{table*}

\subsection{Ablation Studies}

To further analyze the effectiveness of each components, we conduct ablation studies for memory module and personas module. We adopt ChatGLM as our backbone, which is tuned solely using the context of the current session, referred to here as ``Baseline''. Afterward, we separately add ``Event Memory'', ``Agent personas'', and ``User personas'' modules for additional tuning on top of the baseline. The results are presented in Table~\ref{table:msc_ablation}.

The results clearly demonstrate that all modules positively influence long-term dialogue capabilities, with the event memory module contributing the most significant improvements. It is worth noting that although all modules experience a performance decline as the number of sessions increased, the addition of the event memory module results in more stable performance compared to the use of user or agent personas. This highlights the critical role of event memory in maintaining coherence across multiple sessions.


\begin{table}[h]
\centering
\captionsetup{skip=5pt}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}clcccc|ccc@{}}
\toprule
 & & \multicolumn{4}{c|}{\textbf{Extraction}} & \multicolumn{3}{c}{\textbf{Generation}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-9}
\multicolumn{1}{c}{\multirow{-2}{*}{\textbf{}}} & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Extractor}}} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{ACC} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L}  \\
\midrule
& CoT & 5.05 & 2.69 & 25.54 & 61.6 & 5.82 & 1.69 & 16.95 \\
& Tuning & \textbf{8.31} & \textbf{5.65} & \textbf{43.70} & \textbf{77.8} & \textbf{6.12} & \textbf{1.75} & \textbf{17.03} \\

\bottomrule
\end{tabular}
}
\caption{The effect of different extractors on persona extraction and response generation on MSC.}
\label{table:persona}
\end{table}

% \begin{table}[H]
% \centering
% \captionsetup{skip=5pt}
% \caption{The effect of different extractors on persona extraction and response generation on MSC.}
% \label{table:persona}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{@{}clccc@{}}
% \toprule
% \multicolumn{2}{c}{\textbf{Extractor}} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L}  \\
% \midrule
% \multicolumn{5}{l}{\textbf{Extraction}} \\
% \midrule
% & CoT & 5.05 & 2.69 & 25.54 \\
% & Tuning & \textbf{8.31} & \textbf{5.65} & \textbf{43.70} \\
% \midrule
% \multicolumn{5}{l}{\textbf{Generation}} \\
% \midrule
% & CoT & 5.82 & 1.69 & 16.95 \\
% & Tuning & \textbf{6.12} & \textbf{1.75} & \textbf{17.03} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


\subsection{Persona Extraction Analysis}

To explore the effect of different persona extractor, including zero-shot ChatGLM with Chain-of-Thought~\cite{CoT} and ChatGLM tuned on the persona extraction dataset collected from MSC training set, we carry out comparison experiments on two perspectives: Persona Extraction Accuracy and Impact to Response Generation. The results are shown in Table~\ref{table:persona}.


\paragraph{Extraction Accuracy.}

We evaluate the extraction accuracy on the persona extraction dataset collected from MSC testing set, through BLEU-2/3, R-L, and ACC. ACC is to assess the classification accuracy of dividing utterance into ``with personas'' or ``without personas''. The results of extraction in Table~\ref{table:persona} show that the extractor after tuning performs better than CoT on all metrics. The higher BLEU and R-L indicates the tuned extractor performs better capability to extract personas, while higher ACC indicates a stronger capability to distinguish whether personas are contained in an utterance.

\paragraph{Impact to Response Generation.}
In addition, to explore the effect of different persona extractor to the final response generation, we conduct experiments on MSC by comparing the results of zero-shot ChatGLM\textsubscript{LDA} with personas extracted by CoT and tuned extractor, respectively. The Generation results in Table~\ref{table:persona} indicate the tuned extractor performs better in most sessions. As the number of sessions increases, the gap is also constantly expanding, demonstrating tuned extractor is more suitable for long-term dialogue.


%\subsection{Event Perception Analysis}


%\paragraph{Summary Accuracy}

\begin{figure}[h]
    \centering
    \subfigure[Retrieval Mechanism]{
        \includegraphics[width=0.45\linewidth,trim=0 0 0 0,clip]{Figures/ACC_and_Recall.pdf}
        \label{fig:retrieval}
    }
    %\hspace{0.05\linewidth}
    \subfigure[Response Generation]{
        \includegraphics[width=0.45\linewidth,trim=0 0 0 0,clip]{Figures/Model_Evaluation_Chart.pdf}
        \label{fig:generation}
    }
    \caption{The results of human evaluation on retrieval mechanism and response generation.} 
    \label{fig:human}
    \vspace{-0.5cm}
\end{figure}


\subsection{Human Evaluation}

To further explore the performance of LD-Agent in real-life conversation, we adopt human evaluation to evaluate the ability of memory recall and response generation with the results on Figure~\ref{fig:human}.


\paragraph{Retrieval Mechanism Analysis.} Retrieval mechanism plays a crucial role for event memory accurately utilized in long-term dialogue. To evaluate the superiority of topic-based retrieval approach than direct semantic retrieval commonly used in previous methods, we conduct an event memory human evaluation. In the beginning, we initialize a conversation using first four sessions and store event memories for each session into long-term memory bank. In the last session, we let evaluators select relevant memories from long-term memory bank for each utterance as the ground truths. Consequently, we separately utilize direct semantic retrieval and topic-based retrieval to search relevant memories for each utterance, and calculate the accuracy and recall based on human annotations. The results are shown in Figure~\ref{fig:retrieval}. The topic-based retrieval outperforms direct semantic retrieval with significant gap on both ACC and Recall, proving that our retrieval method accurately retrieves relevant memories.


% \begin{figure}[t]
%     \centering
%     \small 
%     \subfloat[Comparison of Different Retrieval Mechanism]{\label{fig:retrieval}
%         \includegraphics[width=0.45\linewidth,trim=0 0 0 0,clip]{Figures/ACC_and_Recall.pdf}
%     }
%     \subfloat[Comparison of Response Generation]
%     {\label{fig:generation}
%         \includegraphics[width=0.45\linewidth,trim=0 0 0 0,clip]{Figures/Model_Evaluation_Chart.pdf}
%     }
%     \caption{The results of human evaluation on retrieval mechanism and response generation.} 
% \label{fig:human}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\linewidth,trim=0 0 0 0,clip]{Figures/ACC_and_Recall.pdf}
%         \label{fig:retrieval}
%     \hfill
%     \includegraphics[width=0.48\linewidth,trim=0 0 0 0,clip]{Figures/Model_Evaluation_Chart.pdf}
%             \label{fig:generation}
%     \caption{The results of human evaluation on retrieval mechanism and response generation.} 
% \label{fig:human}
% \end{figure}


% \begin{figure*}[t]
%     \centering
%     \subfigure[Comparison of Different Retrieval Mechanism]{
%         \includegraphics[width=0.4\linewidth,trim=0 0 0 0,clip]{Figures/ACC_and_Recall.pdf}
%         \label{fig:retrieval}
%     }
%     \hfill
%     \subfigure[Comparison of Response Generation]{
%         \includegraphics[width=0.4\linewidth,trim=0 0 0 0,clip]{Figures/Model_Evaluation_Chart.pdf}
%         \label{fig:generation}
%     }
%     \caption{The results of human evaluation on retrieval mechanism and response generation.} 
%     \label{fig:human}
% \end{figure*}

\begin{table*}[t]
    \centering
    \captionsetup{skip=5pt}
    \resizebox{0.9\textwidth}{!}{%
    \begin{tabular}{@{}lccc|ccc|ccc|ccc@{}}
    \toprule
    & \multicolumn{3}{c}{\textbf{Session 2}} & \multicolumn{3}{c}{\textbf{Session 3}} & \multicolumn{3}{c}{\textbf{Session 4}} & \multicolumn{3}{c}{\textbf{Session 5}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Model}}} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} \\
    \midrule
    \multicolumn{13}{c}{\textbf{MSC}}\\
    \midrule
    Zero-shot & 5.44 & 1.49 & 16.76 & 5.59 & 1.49 & 16.47 & 5.63 & 1.33 & 16.35 & 5.92 & 1.45 & 16.63 \\
    Zero-shot\textsubscript{LDA} & 5.74 & 1.73 & 17.21 & 6.05 & 1.73 & 16.97 & 6.09 & 1.59 & 16.76 & 6.60 & 1.94 & 17.18 \\
    \midrule
    CC-tuning & 5.81 & 1.74 & 18.79 & 6.08 & 1.83 & 18.58 & 5.96 & 1.74 & 18.31 & 5.95 & 1.68 & 18.23 \\
    CC-tuning\textsubscript{LDA} & 7.86 & 3.63 & 21.00 & 7.46 & 3.16 & 20.00 & 7.15 & 2.87 & 19.53 & 7.12 & 2.64 & 19.30 \\
    MSC-tuning & 5.48 & 1.59 & 17.65 & 6.12 & 1.78 & 17.91 & 6.14 & 1.63 & 17.78 & 6.16 & 1.69 & 17.65 \\
    MSC-tuning\textsubscript{LDA} & \textbf{10.70} & \textbf{5.63} & \textbf{23.31} & \textbf{10.03} & \textbf{5.12} & \textbf{21.55 }& \textbf{9.07} & \textbf{4.06} & \textbf{20.19} &\textbf{ 8.96} & \textbf{4.01} & \textbf{19.94} \\
    \midrule
    \multicolumn{13}{c}{\textbf{CC}}\\
    \midrule
    Zero-shot & 9.53 & 4.82 & 22.76 & 9.22 & 4.43 & 22.18 & 9.15 & 4.48 & 22.18 & 8.99 & 4.43 & 22.10 \\
    Zero-shot\textsubscript{LDA} & 8.94 & 4.44 & 21.54 & 8.34 & 4.03 & 21.00 & 8.28 & 3.82 & 20.67 & 8.12 & 3.81 & 20.54 \\
    \midrule
    MSC-tuning & 8.37 & 3.88 & 22.93 & 8.49 & 3.99 & 22.96 & 7.97 & 3.75 & 22.15 & 7.60 & 3.70 & 21.87 \\
    MSC-tuning\textsubscript{LDA} & 21.71 & 15.42 & 34.97 & 20.87 & 14.74 & 34.01 & 19.57 & 13.51 & 32.72 & 18.59 & 12.80 & 31.68 \\
    CC-tuning & 15.89 & 9.90 & 30.59 & 15.97 & 10.06 & 30.27 & 16.10 & 10.31 & 30.54 & 15.10 & 9.34 & 29.43 \\
    CC-tuning\textsubscript{LDA} & \textbf{25.69} & \textbf{19.53} & \textbf{39.67} & \textbf{25.93} & \textbf{19.72} & \textbf{39.15} & \textbf{25.82} & \textbf{19.40} & \textbf{39.05} & \textbf{24.26} & \textbf{18.16} & \textbf{37.61} \\
    \bottomrule
    \end{tabular}
    }
    \caption{The results of cross-domain evaluation on MSC and CC. ``Zero-shot'' indicates the ChatGLM without tuning. ``CC-tuning'' indicates the ChatGLM tuned on CC. ``MSC-tuning'' indicates the ChatGLM tuned on MSC.}
    \label{table:cross_domain}
\end{table*}


\paragraph{Response Generation Analysis.}
To further validate the superiority of LD-Agent in long-term open-domain dialogue tasks, we organize multiple multi-session human-bot conversations on ChatGLM with LD-Agent and w/o LD-Agent. We first initialize a predefined dialogue as the first session for all chatbots. Subsequently, we employ some human evaluators to chat with each chatbot with a time interval from first session. The interactions are evaluated on three aspects: coherence, fluency and engagingness. The results in Figure~\ref{fig:generation} demonstrate the advantages of LD-Agent in long-term real-life dialogue scenarios.

% \begin{table*}[t]
%     \centering
%     \captionsetup{skip=5pt}
%     \caption{The results of cross-domain evaluation on MSC and CC. ``Zero-shot'' indicates the ChatGLM without tuning. ``CC-tuning'' indicates the ChatGLM tuned on CC dataset. ``MSC-tuning'' indicates the ChatGLM tuned on MSC dataset.}
%     \label{table:cross_domain}
%     \resizebox{0.85\textwidth}{!}{%
%     \begin{tabular}{@{}lccc|ccc|ccc|ccc@{}}
%     \toprule
%     & \multicolumn{3}{c}{\textbf{Session 2}} & \multicolumn{3}{c}{\textbf{Session 3}} & \multicolumn{3}{c}{\textbf{Session 4}} & \multicolumn{3}{c}{\textbf{Session 5}} \\
%     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
%     \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Model}}} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} & \textbf{BL-2} & \textbf{BL-3} & \textbf{R-L} \\
%     \midrule
%     \multicolumn{13}{c}{\textbf{MSC}}\\
%     \midrule
%     Zero-shot & 5.44 & 1.49 & 16.76 & 5.59 & 1.49 & 16.47 & 5.63 & 1.33 & 16.35 & 5.92 & 1.45 & 16.63 \\
%     Zero-shot\textsubscript{LDA} & 5.74 & 1.73 & 17.21 & 6.05 & 1.73 & 16.97 & 6.09 & 1.59 & 16.76 & 6.60 & 1.94 & 17.18 \\
%     \midrule
%     CC-tuning & 5.81 & 1.74 & 18.79 & 6.08 & 1.83 & 18.58 & 5.96 & 1.74 & 18.31 & 5.95 & 1.68 & 18.23 \\
%     CC-tuning\textsubscript{LDA} & 7.86 & 3.63 & 21.00 & 7.46 & 3.16 & 20.00 & 7.15 & 2.87 & 19.53 & 7.12 & 2.64 & 19.30 \\
%     MSC-tuning & 5.48 & 1.59 & 17.65 & 6.12 & 1.78 & 17.91 & 6.14 & 1.63 & 17.78 & 6.16 & 1.69 & 17.65 \\
%     MSC-tuning\textsubscript{LDA} & \textbf{10.70} & \textbf{5.63} & \textbf{23.31} & \textbf{10.03} & \textbf{5.12} & \textbf{21.55 }& \textbf{9.07} & \textbf{4.06} & \textbf{20.19} &\textbf{ 8.96} & \textbf{4.01} & \textbf{19.94} \\
%     \midrule
%     \multicolumn{13}{c}{\textbf{CC}}\\
%     \midrule
%     Zero-shot & 9.53 & 4.82 & 22.76 & 9.22 & 4.43 & 22.18 & 9.15 & 4.48 & 22.18 & 8.99 & 4.43 & 22.10 \\
%     Zero-shot\textsubscript{LDA} & 8.94 & 4.44 & 21.54 & 8.34 & 4.03 & 21.00 & 8.28 & 3.82 & 20.67 & 8.12 & 3.81 & 20.54 \\
%     \midrule
%     MSC-tuning & 8.37 & 3.88 & 22.93 & 8.49 & 3.99 & 22.96 & 7.97 & 3.75 & 22.15 & 7.60 & 3.70 & 21.87 \\
%     MSC-tuning\textsubscript{LDA} & 21.71 & 15.42 & 34.97 & 20.87 & 14.74 & 34.01 & 19.57 & 13.51 & 32.72 & 18.59 & 12.80 & 31.68 \\
%     CC-tuning & 15.89 & 9.90 & 30.59 & 15.97 & 10.06 & 30.27 & 16.10 & 10.31 & 30.54 & 15.10 & 9.34 & 29.43 \\
%     CC-tuning\textsubscript{LDA} & \textbf{25.69} & \textbf{19.53} & \textbf{39.67} & \textbf{25.93} & \textbf{19.72} & \textbf{39.15} & \textbf{25.82} & \textbf{19.40} & \textbf{39.05} & \textbf{24.26} & \textbf{18.16} & \textbf{37.61} \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{table*}


\subsection{Generality Analysis}
\label{sec: cross}
We further explore its generality from two perspectives: cross-domain and cross-task capability.

\paragraph{Cross-domain Results.}
The cross-domain capability is crucial for open-domain dialogue task. Poor cross-domain performance, common in models tuned with specific datasets, limits their real-world practicality. To assess our tuned model's real-world potential, we conduct cross-evaluation on MSC and CC, two multi-session datasets with significant domain gaps due to different collection methods, including manual annotation and LLM generation. We first tune ChatGLM on CC and test it on MSC, then reverse the process. The results, shown in Table~\ref{table:cross_domain}, indicate that models tuned on one dataset still performs well on the other dataset, only with a slight performance decrease than the models tuned on the same dataset. Besides, cross-domain tuned models consistently outperform zero-shot models by a significant margin. These experiments highlight the strong cross-domain capability and practical potential of LD-Agent.

\paragraph{Cross-task Results.}
The other capability worth exploring is the transferability of LD-Agent to different dialogue tasks. We explore the effectiveness of our method on multiparty dialogue, a task requires playing multiple roles simultaneously. We conduct our experiments on Ubuntu IRC dataset~\cite{GSN}, a commonly used multiparty dialogue dataset. where our backbone adopts BART~\cite{BART}. We compare our method with some previous multiparty dialogue methods, including GPT-2~\cite{GPT-2}, GSN~\cite{GSN}, HeterMPC\textsubscript{BART}~\cite{HeterMPC}, and BART tuned without prompt. The results are reported at Table~\ref{table:ubuntu} in Appendix.~\ref{sec:add_result}. It can be seen that BART tuned with LD-Agent obtained the state-of-the-art performance in most metrics, outperforming previous multiparty dialogue approach HeterMPC\textsubscript{BART}, which also employs BART as backbone. This well proves the powerful task transferability of LD-Agent.




% \begin{table}[t]
% \centering
% \captionsetup{skip=5pt}
% \caption{Multi-party performance on the Ubuntu IRC benchmark}
% \label{table:ubuntu}
% \begin{tabular}{@{}lccccccc@{}}
% \toprule
% Model                          & \textbf{BL-1} & \textbf{BL-2} & \textbf{BL-3} & \textbf{BL-4} & \textbf{MET} & \textbf{R-L} \\ 
% \midrule
% GPT-2~\cite{GPT-2} & 10.37  & 3.60   & 1.66   & 0.93   & 4.01   & 9.53    \\
% GSN~\cite{GSN} & 10.23  & 3.57   & 1.70   & 0.97   & 4.10   & 9.91    \\
% HeterMPC\textsubscript{BART}~\cite{HeterMPC} & 12.26  & 4.80   & \textbf{2.42}   & \textbf{1.49}   & 4.94   & 11.20   \\
% BART~\cite{BART} & 11.25   & 4.02   & 1.78   & 0.95   & 4.46   & 9.90  \\
% \midrule
% %BART-Base  & 13.40   & 4.87   & 2.26   & 1.26   & 5.06   & 12.00    \\
% BART\textsubscript{LDA} & \textbf{14.40}   & \textbf{4.92}   & 2.07   & 1.00   & \textbf{5.30}   & \textbf{12.28}  \\
% %\hspace{3mm}Fine-tuning Only (FO)   & 11.47  & 5.11   & 2.98   & 2.11   & 5.23   & 11.31   \\
% \bottomrule
% \end{tabular}
% \end{table}


==> chapters/5_conclusion_pre.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we delved into the long-term open-domain dialogue agent to meet real-life chatbot demands for long-term companionship and personalized interactions. We introduced a model-agnostic long-term dialogue agent framework, LD-Agent, which comprehensively considers both historical events and user-agent personas to support coherent and consistent conversation. Our framework, decomposed into three learnable modules, significantly enhances adaptability and transferability. Extensive experiments demonstrated LD-Agent's strong capability in handling long-term dialogue tasks, showcasing its practicality across multiple benchmarks, models, and tasks.


